Classification of Chinese Handwritten Numbers with Labeled Projective Dictionary Pair Learning

Dictionary learning is a cornerstone of image classification. We set out to address a longstanding challenge in using dictionary learning for classification; that is to simultaneously maximise the discriminability and sparse-representability power of the learned dictionaries. Upon this premise, we designed class-specific dictionaries incorporating three factors: discriminability, sparsity and classification error. We integrated these metrics into a unified cost function and adopted a new feature space, i.e., histogram of oriented gradients (HOG), to generate the dictionary atoms. The rationale of using HOG features for designing the dictionaries is their strength in describing fine details of crowded images. The results of applying the proposed method in the classification of Chinese handwritten numbers demonstrated enhanced classification performance $(\sim98\%)$ compared to state-of-the-art deep learning techniques (i.e., SqueezeNet, GoogLeNet and MobileNetV2), but with a fraction of parameters. Furthermore, combination of the HOG features with dictionary learning enhances the accuracy by $11\%$ compared to the case where only pixel domain data are used. These results were supported when the proposed method was applied to both Arabic and English handwritten number databases.

==> LpDPL-v1 <==
% Generated by IEEEtran.bst, version: 1.14 (2015/08/26)
\begin{thebibliography}{10}
\providecommand{\url}[1]{#1}
\csname url@samestyle\endcsname
\providecommand{\newblock}{\relax}
\providecommand{\bibinfo}[2]{#2}
\providecommand{\BIBentrySTDinterwordspacing}{\spaceskip=0pt\relax}
\providecommand{\BIBentryALTinterwordstretchfactor}{4}
\providecommand{\BIBentryALTinterwordspacing}{\spaceskip=\fontdimen2\font plus
\BIBentryALTinterwordstretchfactor\fontdimen3\font minus
  \fontdimen4\font\relax}
\providecommand{\BIBforeignlanguage}[2]{{%
\expandafter\ifx\csname l@#1\endcsname\relax
\typeout{** WARNING: IEEEtran.bst: No hyphenation pattern has been}%
\typeout{** loaded for the language `#1'. Using the pattern for}%
\typeout{** the default language instead.}%
\else
\language=\csname l@#1\endcsname
\fi
#2}}
\providecommand{\BIBdecl}{\relax}
\BIBdecl

\bibitem{10.3389/fncom.2015.00099}
P.~Diehl and M.~Cook, ``Unsupervised learning of digit recognition using
  spike-timing-dependent plasticity,'' \emph{Frontiers in Computational
  Neuroscience}, vol.~9, p.~99, 2015.

\bibitem{qiao2018adaptive}
J.~Qiao, G.~Wang, W.~Li, and M.~Chen, ``An adaptive deep q-learning strategy
  for handwritten digit recognition,'' \emph{Neural Networks}, vol. 107, pp.
  61--71, 2018.

\bibitem{9110900}
S.~{Aly} and S.~{Almotairi}, ``Deep convolutional self-organizing map network
  for robust handwritten digit recognition,'' \emph{IEEE Access}, vol.~8, pp.
  107\,035--107\,045, 2020.

\bibitem{farsiNumber}
M.~Akhlaghi and V.~Ghods, ``Farsi handwritten phone number recognition using
  deep learning,'' \emph{SN Applied Sciences}, vol.~2, no.~3, April 2020.

\bibitem{yu2015handwritten}
N.~Yu, P.~Jiao, and Y.~Zheng, ``Handwritten digits recognition base on improved
  lenet5,'' in \emph{The 27th Chinese Control and Decision Conference (2015
  CCDC)}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2015, pp. 4871--4875.

\bibitem{lauer2007trainable}
F.~Lauer, C.~Y. Suen, and G.~Bloch, ``A trainable feature extractor for
  handwritten digit recognition,'' \emph{Pattern Recognition}, vol.~40, no.~6,
  pp. 1816--1824, 2007.

\bibitem{choudhury2018handwritten}
A.~Choudhury, H.~S. Rana, and T.~Bhowmik, ``Handwritten bengali numeral
  recognition using hog based feature extraction algorithm,'' in \emph{2018 5th
  International Conference on Signal Processing and Integrated Networks
  (SPIN)}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2018, pp. 687--690.

\bibitem{9092067}
S.~{Hamida}, B.~{Cherradi}, and H.~{Ouajji}, ``Handwritten arabic words
  recognition system based on hog and gabor filter descriptors,'' in \emph{2020
  1st International Conference on Innovative Research in Applied Science,
  Engineering and Technology (IRASET)}, 2020, pp. 1--4.

\bibitem{9084035}
S.~{Tajrean} and M.~{Abu Yousuf}, ``Handwritten bengali number detection using
  region proposal network,'' in \emph{2019 International Conference on Bangla
  Speech and Language Processing (ICBSLP)}, 2019, pp. 1--6.

\bibitem{luo2019multi}
X.~Luo, Y.~Xu, and J.~Yang, ``Multi-resolution dictionary learning for face
  recognition,'' \emph{Pattern Recognition}, vol.~93, pp. 283--292, 2019.

\bibitem{8563234}
W.~{Wang}, J.~{Zhang}, J.~{Du}, Z.~{Wang}, and Y.~{Zhu}, ``Denseran for offline
  handwritten chinese character recognition,'' in \emph{2018 16th International
  Conference on Frontiers in Handwriting Recognition (ICFHR)}, 2018, pp.
  104--109.

\bibitem{9085435}
Z.~{Li}, Y.~{Xiao}, Q.~{Wu}, M.~{Jin}, and H.~{Lu}, ``Deep template matching
  for offline handwritten chinese character recognition,'' \emph{The Journal of
  Engineering}, vol. 2020, no.~4, pp. 120--124, 2020.

\bibitem{8869841}
J.~{Zhang}, H.~{Bi}, Y.~{Chen}, M.~{Wang}, L.~{Han}, and L.~{Cai},
  ``Smarthandwriting: Handwritten chinese character recognition with
  smartwatch,'' \emph{IEEE Internet of Things Journal}, vol.~7, no.~2, pp.
  960--970, 2020.

\bibitem{DLbook/3265797}
B.~Dumitrescu and P.~Irofti, \emph{Dictionary Learning Algorithms and
  Applications}, 1st~ed.\hskip 1em plus 0.5em minus 0.4em\relax Springer
  Publishing Company, Incorporated, 2018.

\bibitem{wright2008robust}
J.~Wright, A.~Y. Yang, A.~Ganesh, S.~S. Sastry, and Y.~Ma, ``Robust face
  recognition via sparse representation,'' \emph{IEEE transactions on pattern
  analysis and machine intelligence}, vol.~31, no.~2, pp. 210--227, 2008.

\bibitem{huang2007sparse}
K.~Huang and S.~Aviyente, ``Sparse representation for signal classification,''
  in \emph{Advances in neural information processing systems}, 2007, pp.
  609--616.

\bibitem{aharon2006k}
M.~Aharon, M.~Elad, and A.~Bruckstein, ``K-svd: An algorithm for designing
  overcomplete dictionaries for sparse representation,'' \emph{IEEE
  Transactions on signal processing}, vol.~54, no.~11, pp. 4311--4322, 2006.

\bibitem{shin2012sparse}
Y.~Shin, S.~Lee, J.~Lee, and H.-N. Lee, ``Sparse representation-based
  classification scheme for motor imagery-based brain--computer interface
  systems,'' \emph{Journal of neural engineering}, vol.~9, no.~5, p. 056002,
  2012.

\bibitem{10.5555/2981780.2981909}
J.~Mairal, F.~Bach, J.~Ponce, G.~Sapiro, and A.~Zisserman, ``Supervised
  dictionary learning,'' in \emph{Proceedings of the 21st International
  Conference on Neural Information Processing Systems}, ser. NIPS’08.\hskip
  1em plus 0.5em minus 0.4em\relax Red Hook, NY, USA: Curran Associates Inc.,
  2008, p. 1033–1040.

\bibitem{fulkerson2008localizing}
B.~Fulkerson, A.~Vedaldi, and S.~Soatto, ``Localizing objects with smart
  dictionaries,'' in \emph{European Conference on Computer Vision}.\hskip 1em
  plus 0.5em minus 0.4em\relax Springer, 2008, pp. 179--192.

\bibitem{winn2005object}
J.~Winn, A.~Criminisi, and T.~Minka, ``Object categorization by learned
  universal visual dictionary,'' in \emph{Tenth IEEE International Conference
  on Computer Vision (ICCV'05) Volume 1}, vol.~2.\hskip 1em plus 0.5em minus
  0.4em\relax IEEE, 2005, pp. 1800--1807.

\bibitem{zhang2010discriminative}
Q.~Zhang and B.~Li, ``Discriminative k-svd for dictionary learning in face
  recognition,'' in \emph{2010 IEEE Computer Society Conference on Computer
  Vision and Pattern Recognition}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE,
  2010, pp. 2691--2698.

\bibitem{jiang2011learning}
Z.~Jiang, Z.~Lin, and L.~S. Davis, ``Learning a discriminative dictionary for
  sparse coding via label consistent k-svd,'' in \emph{CVPR 2011}.\hskip 1em
  plus 0.5em minus 0.4em\relax IEEE, 2011, pp. 1697--1704.

\bibitem{jiang2013label}
Z.~{Jiang}, Z.~{Lin}, and L.~S. {Davis}, ``Label consistent k-svd: Learning a
  discriminative dictionary for recognition,'' \emph{IEEE Transactions on
  Pattern Analysis and Machine Intelligence}, vol.~35, no.~11, pp. 2651--2664,
  2013.

\bibitem{8745700}
W.~{Tang}, A.~{Panahi}, H.~{Krim}, and L.~{Dai}, ``Analysis dictionary learning
  based classification: Structure for robustness,'' \emph{IEEE Transactions on
  Image Processing}, vol.~28, no.~12, pp. 6035--6046, 2019.

\bibitem{8038251}
Z.~{Zhang}, W.~{Jiang}, J.~{Qin}, L.~{Zhang}, F.~{Li}, M.~{Zhang}, and
  S.~{Yan}, ``Jointly learning structured analysis discriminative dictionary
  and analysis multiclass classifier,'' \emph{IEEE Transactions on Neural
  Networks and Learning Systems}, vol.~29, no.~8, pp. 3798--3814, 2018.

\bibitem{gu2014projective}
S.~Gu, L.~Zhang, W.~Zuo, and X.~Feng, ``Projective dictionary pair learning for
  pattern classification,'' in \emph{Advances in neural information processing
  systems}, 2014, pp. 793--801.

\bibitem{ameri2016projective}
R.~Ameri, A.~Pouyan, and V.~Abolghasemi, ``Projective dictionary pair learning
  for eeg signal classification in brain computer interface applications,''
  \emph{Neurocomputing}, vol. 218, pp. 382--389, 2016.

\bibitem{abolghasemi2018incoherent}
V.~Abolghasemi, M.~Chen, A.~Alameer, S.~Ferdowsi, J.~Chambers, and
  K.~Nazarpour, ``Incoherent dictionary pair learning: Application to a novel
  open-source database of chinese numbers,'' \emph{IEEE Signal Processing
  Letters}, vol.~25, no.~4, pp. 472--476, 2018.

\bibitem{7779008}
S.~{Tariyal}, A.~{Majumdar}, R.~{Singh}, and M.~{Vatsa}, ``Deep dictionary
  learning,'' \emph{IEEE Access}, vol.~4, pp. 10\,096--10\,109, 2016.

\bibitem{8658671}
H.~{Tang}, H.~{Wei}, W.~{Xiao}, W.~{Wang}, D.~{Xu}, Y.~{Yan}, and N.~{Sebe},
  ``Deep micro-dictionary learning and coding network,'' in \emph{2019 IEEE
  Winter Conference on Applications of Computer Vision (WACV)}, 2019, pp.
  386--395.

\bibitem{1446833}
\BIBentryALTinterwordspacing
B.~Tolooshams, A.~H. Song, S.~Temereanca, and D.~Ba, ``Convolutional dictionary
  learning based auto-encoders for natural exponential-family distributions,''
  2020. [Online]. Available: \url{https://arxiv.org/abs/1907.03211}
\BIBentrySTDinterwordspacing

\bibitem{DataBase2019}
``Handwritten chinese numbers,'' Accessed: 29-Nov-2019.

\bibitem{AHD}
``The arabic handwritten digits databases,''
  \url{http://datacenter.aucegypt.edu/shazeem/}, accessed: 2020-09-10.

\bibitem{Hull1994}
J.~J. Hull, ``A database for handwritten text recognition research,''
  \emph{IEEE Transactions on pattern analysis and machine intelligence},
  vol.~16, pp. 550--554, 1994.

\bibitem{otsu1979threshold}
N.~Otsu, ``A threshold selection method from gray-level histograms,''
  \emph{IEEE transactions on systems, man, and cybernetics}, vol.~9, no.~1, pp.
  62--66, 1979.

\bibitem{Freeman1995OrientationHF}
W.~T. Freeman and M.~Roth, ``Orientation histograms for hand gesture
  recognition,'' 1995.

\bibitem{goldstein2014fast}
T.~Goldstein, B.~O'Donoghue, S.~Setzer, and R.~Baraniuk, ``Fast alternating
  direction optimization methods,'' \emph{SIAM Journal on Imaging Sciences},
  vol.~7, no.~3, pp. 1588--1623, 2014.

\bibitem{ramirez2010classification}
I.~Ramirez, P.~Sprechmann, and G.~Sapiro, ``Classification and clustering via
  dictionary learning with structured incoherence and shared features,'' in
  \emph{2010 IEEE Computer Society Conference on Computer Vision and Pattern
  Recognition}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2010, pp.
  3501--3508.

\bibitem{sandler2018mobilenetv2}
M.~Sandler, A.~Howard, M.~Zhu, A.~Zhmoginov, and L.-C. Chen, ``Mobilenetv2:
  Inverted residuals and linear bottlenecks,'' in \emph{Proceedings of the IEEE
  conference on computer vision and pattern recognition}, 2018, pp. 4510--4520.

\bibitem{szegedy2015going}
C.~Szegedy, W.~Liu, Y.~Jia, P.~Sermanet, S.~Reed, D.~Anguelov, D.~Erhan,
  V.~Vanhoucke, and A.~Rabinovich, ``Going deeper with convolutions,'' in
  \emph{Proceedings of the IEEE conference on computer vision and pattern
  recognition}, 2015, pp. 1--9.

\bibitem{iandola2016squeezenet}
F.~N. Iandola, S.~Han, M.~W. Moskewicz, K.~Ashraf, W.~J. Dally, and K.~Keutzer,
  ``Squeezenet: Alexnet-level accuracy with 50x fewer parameters and< 0.5 mb
  model size,'' \emph{arXiv preprint arXiv:1602.07360}, 2016.

\bibitem{deng2009imagenet}
J.~Deng, W.~Dong, R.~Socher, L.-J. Li, K.~Li, and L.~Fei-Fei, ``Imagenet: A
  large-scale hierarchical image database,'' in \emph{2009 IEEE conference on
  computer vision and pattern recognition}.\hskip 1em plus 0.5em minus
  0.4em\relax Ieee, 2009, pp. 248--255.

\bibitem{ArabicCNN}
A.~El-Sawy, H.~EL-Bakry, and M.~Loey, ``Cnn for handwritten arabic digits
  recognition based on lenet-5,'' in \emph{Proceedings of the International
  Conference on Advanced Intelligent Systems and Informatics 2016}, A.~E.
  Hassanien, K.~Shaalan, T.~Gaber, A.~T. Azar, and M.~F. Tolba, Eds.\hskip 1em
  plus 0.5em minus 0.4em\relax Cham: Springer International Publishing, 2017,
  pp. 566--575.

\end{thebibliography}

